On the Impact of Temporal Concept Drift on Model Explanations

Explanation faithfulness of model predictions in natural language processing is typically evaluated on held-out data from the same temporal distribution as the training data (i.e. synchronous settings). While model performance often deteriorates due to temporal variation (i.e. temporal concept drift), it is currently unknown how explanation faithfulness is impacted when the time span of the target data is different from the data used to train the model (i.e. asynchronous settings). For this purpose, we examine the impact of temporal variation on model explanations extracted by eight feature attribution methods and three select-then-predict models across six text classification tasks. Our experiments show that (i)faithfulness is not consistent under temporal variations across feature attribution methods (e.g. it decreases or increases depending on the method), with an attention-based method demonstrating the most robust faithfulness scores across datasets; and (ii) select-then-predict models are mostly robust in asynchronous settings with only small degradation in predictive performance. Finally, feature attribution methods show conflicting behavior when used in FRESH (i.e. a select-and-predict model) and for measuring sufficiency/comprehensiveness (i.e. as post-hoc methods), suggesting that we need more robust metrics to evaluate post-hoc explanation faithfulness.

==> todo.tex <==
6 June

1. short intro 
2. related work
    - short
    - remove 2.3 (DONE)
3. 3.1 change to para 
4. experiment set up
    - add for evaluation as 2.3 removed
5. fig 2, change order
6. fig 3, change to scatter (DONE)




others:
- change to use select-then-predict (DONE)
- table 1 change to 1/3 size (DONE)
- table 2 to appendix (DONE)
- add DEEPLIFT AND GRADIENT FOR FRESH (RUNNING)
 * agnews, yelp done
 * digimu pantry xfact factcheck
 
 
 
 
------------------
 
Structure I was thinking about
1. Posthoc pure
2. Select-then-predict pure
3. Quantitative analysis
    3.1 fresh vs posthoc --> what do we see, why is it different, possible reasons
    3.2 possible reasons of temporal variation affecting sufficiency comprehensiveness?
    3.3 explanation game thing
5. Discussion 
    5.1 Sufficiency and Comprehensiveness are misleading in temporal ...
    5.2 Evaluate faithfulness out-of-time with 'explanation game'
    5.3 Select-then-predict work
    5.4 temporal performance depends on ..... 
    
TODO:
* check YELP hyperparams
* find excuse for XFACT and FACTCHECK --> low datapoints - high classes

RESULTS:

** POSTHOC **

\begin{enumerate}
    \item No single feature attribution performs ALWAYS above the random baseline. Scaled attention looks like its the most sufficient and comprehensive overall
    \item There is no clear pattern for explanation sufficiency and comprehensiveness in out-of-time settings. Sometimes increases, for example in .... Sometimes decreases ... and there is no clear relation to the model performance.
    \item We argue that sufficiency and comprehensiveness can be misleading when used to evaluate explanations in out-of-time settings for this reason as their behaviour is erratic. We are not convinced that we can rely on these metrics when temporal variations occur.
    \item to investigate further in Section ... we examine possible factors of this. We also explore whether using the ``explanation game'' evaluation approach yields more reliable results in Section or Appendix ... 
\end{enumerate}

** SELECT-then-PREDICT ** 
\begin{enumerate}
    \item FRESH with alpha alpha performs actually comparable to full text BERT and CAN be used. Same trend. 
    \item FRESH performance HIGHLY depends on feature attribution (fig. 4)
    \item SOME feature attributions do not seem to impact model performance or be affected by temporal variations. In only a few tasks (xfact)
    \item HARDKUMA and SPECTRA perform well when we have a lot of data on simple tasks. However, on more complex tasks with less datapoints (xfact, factcheck) we see their performance drop. 
    \item HOWEVER, if HARDKUMA perform well (close to LSTM) in-domain FULL then you can expect them to work well with temporal variations. FOR SPECTRA NO.
\end{enumerate}

ANALYSIS AND DISUSSION

** FRESH PERFORMS WELL - SUFF and COMP no? **
\begin{enumerate}
    \item Deeplift performs bad as post-hoc, great as FRESH in some cases. Why? We think that SUFF and comp are very misleading out-of-domain and sometimes in domain. OPTIONAL: For this purpose we do explanation game to align everything. 
    \item SECTION: Also, does the drop in FRESH performance, HARDKUMA performance in out-of-time depend on corpus similarity or time variation? 
    We hypothesize that one of the reasons why faithfulness (with select-then-predict or post-hoc) drops in out-of-domain might be because of the high difference in corpus similarity?
    \item SECTION : Does performance of explanations depend on time difference between train and test? Test split to 10\% - 100\%. Correlate distance from training data to corpus similarity.
\end{enumerate}

Explanations GAME:
Explanations -> Classifier
Classifier can be anything: BERT (FRESH), LSTM (HARDKUMA, SPECTRA)
Explanations from feature attribution with LSTM on top


---------
YELP after hyperparameter, using the current version on jade, not the old run folder one. 
---------



\begin{comment}
agnews:    most above random baseline, especially on comprehensive. no pattern between asyd and synd
xfact:     random, most comprehensiveness above random baseline
**factcheck: SynD > AsyD both suf and comp, most above random baseline
**digimu:    SynD slightly > AsyD both suf and comp, except gradients-based feature attributions on comprehensiveness; lest suff above random
**pantry:    SynD slightly > AsyD both suf and comp, except gradients-based feature attributions on comprehensiveness
yelp:      random, most above baseline except 

no single gradients-based features above random cross all tasks. 
We consider several potential factors for explanation performance in asynchronous settings. 
** corpus similarity: SynD train -- SynD test, SynD train -- AsyD test where SynD train -- SynD test is taken as the baseline
** temporal distance: SynD train -- SynD test, SynD train -- AsyD test where SynD train -- SynD test is taken as the baseline
** temporal density: average number of data points for one single day: SynD train -- SynD test, SynD train -- AsyD test where SynD train -- SynD test is taken as the baseline 
** sentiment distribution: SynD train, SynD test, AsyD1 test, AsyD2 test (limitation, how we measure the sentiment) 
** label distribution (multi label?)

\end{comment}




Our standard for a reliable feature attribution method in asynchronous settings come in two-folds: its faithfulness is above random baseline, and it demonstrates smaller fluctuations across chronological splits as it indicates a small impact under temporal drift. 
